Similarity is Not All You Need: Endowing Retrieval Augmented Generation with Multi Layered Thoughts

In recent years, large language models (LLMs) have made remarkable achievements in various domains. However, the untimeliness and cost of knowledge updates coupled with hallucination issues of LLMs have curtailed their applications in knowledge intensive tasks, where retrieval augmented generation (RAG) can be of help. Nevertheless, existing retrieval augmented models typically use similarity as a bridge between queries and documents and follow a retrieve then read procedure. In this work, we argue that similarity is not always the panacea and totally relying on similarity would sometimes degrade the performance of retrieval augmented generation. To this end, we propose MetRag, a Multi layEred Thoughts enhanced Retrieval Augmented Generation framework. To begin with, beyond existing similarity oriented thought, we embrace a small scale utility model that draws supervision from an LLM for utility oriented thought and further come up with a smarter model by comprehensively combining the similarity and utility oriented thoughts. Furthermore, given the fact that the retrieved document set tends to be huge and using them in isolation makes it difficult to capture the commonalities and characteristics among them, we propose to make an LLM as a task adaptive summarizer to endow retrieval augmented generation with compactness-oriented thought. Finally, with multi layered thoughts from the precedent stages, an LLM is called for knowledge augmented generation. Extensive experiments on knowledge-intensive tasks have demonstrated the superiority of MetRag.

==> rebuttal_backup_for_later_comparison.tex <==
\clearpage
\appendix
\section{Rebuttal}
\subsection{Reply to Reviewer HsYx}
\noindent \textbf{W1. About utility} ``\emph{This paper does not provide a specific definition of utility. The similarity is usually based on relevance labels, while the utility is more like usefulness. This paper models utility by the normalization of the probability of generating correct answers with a specific LLM. The authors use an LLM to generate the supervision signal for utility. However, I did not find what LLM they have used. What is the impact of different LLMs on utility modeling? The authors may need to test at least two different LLMs. For some questions, LLM can answer them based on its own knowledge. In this case, a useful passage for these questions is not useful for LLM to answer these questions. Then, are these passages with low utility or high utility?}''

\noindent \textbf{A} Thank you for your nice comments and we apologize for the confusion. We are committed to resolving the issue promptly as outlined below:
\begin{itemize}[leftmargin=*]
    \item \emph{Definition of the utility.} In this paper, we define the utility of one document \wrt a question by its usefulness in assisting an LLM to answer this question, which is modelled by the normalization of the probability of generating correct answers with a specific LLM. In Sec.xxx, we have mentioned the choice of the LLM, \ie ``train our model in different stages with Llama2$_{\textsc{13b}}$ as base LLM''. To avoid misunderstanding, we will revise it in the final version as ``train our model in different stages (including utility model, task-adaptive summarizer and the final LLM for generating answers) with Llama2$_{\textsc{13b}}$ as base LLM''. Owing to time limitation, we have been unable to complete the experiments exploring the impact of different LLMs on utility modeling, but we are actively working on it. We intend to incorporate the relevant experimental findings into the final version of our work.

    \item \emph{When a passage is not useful for LLMs.}
\end{itemize}


In this paper, we define the utility of one document \wrt a question by its usefulness in assisting an LLM to answer this question and we model it by the normalization of the probability of generating correct answers with a specific LLM. As for the choice of the LLM, we only mention it in the Training details of Settings by saying "train our model in different stages with Llama2$_{\textsc{13b}}$ as base LLM". To avoid disambiguation, we will revise this to "train our model in different stages (including utility model, task-adaptive summarizer and the final LLM for generating answers) with Llama2$_{\textsc{13b}}$ as base LLM". Due to the time limitation, we cannot finish all experiments by incorporating other LLMs for testing but we are working on it for improving our work.

As for the second question, when a passage is not useful for an LLM to answer a question, it is of low utility in our definition. In lines 275-279 of Section \ref{sec:combination}, we add an interesting mechanism in designing the utility model by adding an empty string, so that the utility model is equipped with the ability to judge whether introducing a document for a query can promote the utility or not thus achieving selective retrieval. Furthermore, we have discussed the impact of this mechanism in Impact of selective retrieval in Section \label{sec:exp} that for 20.9\% quries the utility model ranks the empty string higher than other retrieved documents, which suggests that we should pay more attention to the innate knowledge of a given LLM when conducting retrieval and we believe that our work has provided an easy and plausible solution.

\noindent \textbf{Comment 2} Some details about the methods and baselines need to be clarified.

\noindent \textbf{Comment 2-1} It is unclear what the teacher model in the summarization task is. Line 135 shows "e.g., GPT4" while line 327 shows "e.g., ChatGPT".

\noindent \textbf{Response 2-1} Thank you for your comments and we are sorry for the confusing statements. The teacher model in the summarization task is GPT4, and we have modified the inconsistent examples in these lines and further specify the teacher model in the Training details of Settings.

\noindent \textbf{Comment 2-2} It is unclear what the I() in equation (5) is. The authors said that "we simply implement it as simple concatenation". Perhaps I misunderstood. Do the authors mean obtaining the final ranking score through the concatenation of similarity and utility scores? How to do this?

\noindent \textbf{Response 2-2} Thank you for your comments and we apologize for the disambiguation. For the final documents, due to the reason that the similarity score and the utility score is not comparable, with the given parameter $k$ being the total retrieved documents limits, we simply concat the top $\left \lfloor k/2 \right \rfloor$ documents measured by similarity and top $\left \lfloor k/2 \right \rfloor$ documents measured by utility  and leave other more sophisticated approaches for future work.

\noindent \textbf{Comment 2-3} For baselines with retrievals, the author says "an LM (e.g., Llama27B,13B) generates output given the query prepended with the top retrieved documents.". Is the top retrieved document here only considering the similarity? Why hasn't the result of ChatGPT with retrieval been reported?

\noindent \textbf{Response 2-3} Thank you for your comments. As for baselines with retrievals, the top retrieved documents here only consider the similarity for the reason that in a typical retrieval-augmented scenario usually only the similarity rather than utility is considered, and we hope to showcase the power of utility-based thought in our experiment. 
\begin{table}[t]\centering
\caption{Comparison to ChatGPT with Retrieval} 
\setlength{\tabcolsep}{0.5mm}{
\label{tab:compare_with_chatgot}
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\multirow{2}{*}{Methods}
& \multicolumn{2}{c|}{NQ} 
& \multicolumn{2}{c|}{TriviaQA} 
& \multicolumn{2}{c|}{HotpotQA} 
& \multicolumn{2}{c}{PopQA} 
\\    
\cmidrule{2-9}
%\midrule
 {} 
 & {EM} & {F1} 
 & {EM} & {F1} 
 & {EM} & {F1} 
 & {EM} & {F1}\\ 
\midrule 
{ChatGPT} 
& {51.5} & {54.5} 
& {72.3} & {73.2} 
& {39.9} & {45.7}   
& {64.4} & {63.6}   \\
\midrule
{\model} 
& {49.6} & {53.9} 
& {\textbf{74.8}} & {\textbf{78.7}} 
& {\textbf{42.2}} & {\textbf{51.9}} 
& {58.8} & {61.5}  \\
\bottomrule
\end{tabular}}
\end{table}

As for retrieval with ChatGPT, we have added corresponding experiments, and the experimental results are listed in Table \ref{tab:compare_with_chatgot}.
As we can see from this table, our {\model} can surpass the 175B ChatGPT in half of the evaluated datasets (\ie TriviaQA and HotpotQA) which contribute 78.9\% questions in testing by a large margin, which further illustrates that great performance can be achieved even with small-scale LMs.


\noindent \textbf{Comment 3} C1. The abbreviations C1 and C2 in the last paragraph of the Introduction are not used elsewhere in the paper.
C2. All figures and tables should be put at the top of the page.
C3. In line 334, the $I_s^q$ should be $I_q^s$.

\noindent \textbf{Response 3} Thank you for your nice comments. As for C1 and C2 in the Introduction, it corresponds to the challenges mentioned in the third paragraph of the Introduction. To avoid disambiguation, we have replaced the i) and ii) in this paragraph to C1 and C2. As for all the figures and tables in this paper, we have reorganized to the top of each corresponding page. At last, the typo in line 334 has been fixed.

\subsection{Reply to Reviewer sCoY}
\noindent \textbf{Comment 1} I have some concerns about the novelty of some of the proposed components. For instance, utilizing reader's feedback to train a retrieval model has been studied since 2020 in the exact same method but using a smaller language model (https://arxiv.org/abs/2010.10999) or even more complicated approaches (https://arxiv.org/abs/2012.04584, https://arxiv.org/abs/2208.03299). Additionally, the idea of summarization for RAG has also been studied (https://arxiv.org/abs/2310.04408); however, this paper uses DPO style optimization, which is definitely novel.

\noindent \textbf{Response 1} Thank you for your comments. We would like to explain this from the following two perspectives. 
As for utilizing reader's feedback to train the retrieval model, we have carefully reviewed the papers you provided and other similar papers, from which we can conclude that 1) though there are other approaches utilized LLM's power to improve retriever, they totally rely on LLM by either introducing all the top documents after ranking or only utilize the top one for further inference or not distinguishing whether retrieval is necessary, 2) they totally rely on the power of LLMs in making decision, while we believe in LLM's power under many circumstances but still recognize that there are certain insufficiencies in it and further introduces the similarity-oriented thought to make up for these insufficiencies and justifies these design in our experiments.
As for summarization for RAG, we have carefully reviewed paper you refer to, which is also included in our experiments as baselines, however, it designs intricate samples and performs distillation without further aligning strategy for performance boosting, which downgrades its performance in applications. Instead, we perform alignment in our summarizer training for enhancing performance.

\noindent \textbf{Comment 2} This paper only focuses on the datasets where the expected output is short (like an answer to a trivia question). It would be nice if we could see the results on a long-form QA dataset such as ELI5.

\noindent \textbf{Response 2} Thank you for your nice suggestions. We conduct experiments on these QA datasets by carefully cross-examining the experimental settings and summaries of many works such as 1) When Not to Trust Language Models: Investigating Effectiveness of Parametric and Non-Parametric Memories, 2) Self-rag: Learning to retrieve, generate, and critique through self-reflection, 3) RECOMP: improving retrieval-augmented lms with compression and selective augmentation, 4) Llama 2: Open Foundation and Fine-Tuned Chat Models and so on to make sure that the datasets we evaluate are widely-used. We sincerely thank you for your nicely suggestions to involve long-form QA dataset and we are conducting research on the relevant data and corresponding papers for 
supplementary experiments. However, due to the time limitation of the rebuttal period, we cannot finish all these experiments but we are working on it for improving our work.

\noindent \textbf{Comment 3} This paper does not come with a section on limitations, which was required for all submitted papers.

\noindent \textbf{Response 3} Thank you for your nice suggestions. We have pointed out our limitations in Section 4 and Section \ref{sec:con} but haven't organized them into a separate section. Hence we would add a follow-up section to discuss the related issues by including the following contents:

\textit{In this work, we have proposed an interesting mechanism 
by adding an empty string when optimizing the utility model 
to leverage the knowledge of LLMs to achieve selective retrieval. 
We would find that many of queries are commonsense knowledge 
that has been memorized in LLMs' parameters and we can easily call 
an LLM for the required answer instead of retrieval, which
illustrates that in retrieval-augmented generation, despite 
the further knowledge external corpus introduces, the knowledge 
stored in LLMs' parameters is worth investigation and our proposed 
approach provides an easy and plausible solution to decide if 
there is need for retrieval. However, this design still has certain 
limitations, \ie the LLM used for end task needs to be 
the same or stronger than the one utilized during utility model 
training, otherwise this mechanism may not work. Besides, our work 
opens up a fresh perspective to reconsider retrieval-augmented 
generation, but we have not yet resolved the situation when the 
retrieved context length is beyond limitation in generation, \eg 
legal or medical documents, which is left as future work.}



\subsection{Reply to Reviewer bS2v}
\noindent \textbf{Comment 1} For Example, the authors mentioned “Though LLMs can serve as data annotators and come up with high quality corpus for model training and have demonstrated their tremendous capability in many circumstances, the innate uncontrollable and instability characteristics would sometimes deteriorate the performance.” I don’t think the researchers who work on LLM autoeval would fully agree with the statement. Also, even the authors themselves used LLM to critique and improve their model (although they later combine results for better stability).

\noindent \textbf{Response 1} Thank you for your comments. Despite their tremendous power in diverse tasks such as question answering, translation and so on, the hallucinations and uncontrollable issues of LLMs have been discussed in many research works (\eg 1) When Not to Trust Language Models: Investigating Effectiveness of Parametric and Non-Parametric Memories, 2) Retrieval-Augmented Generation for Large Language Models: A Survey), which has limited the applications of LLMs in certain areas such as medical, finance and so on. We fully admit the power of LLMs in so many situations, however, we also think that we need task "safety measures" when using LLMs.


\noindent \textbf{Comment 2} The authors mentioned “With high-quality retrieved documents, to reduce the burden that dozens of documents impose on LLMs and better capture the commonalities and characteristics between retrieved documents, document summarization is plausible.” Then in the whole paper, the authors used summarization as the default setting. Actually, some previous research found that a combination of summary and raw retrieved results could achieve better performance.

\noindent \textbf{Response 2} We use summarization as the default setting for two reasons: 1) We hope that through summarization we can abstract enough useful information for the downstream tasks and in turn avoid using a dozen of retrieved information which might causes distraction for LLMs, which we have examined its rationality in our ablation study that compared to using retrieved all information for downstream tasks, only incorporating the summarization information can improve the EM and F1 metrics for these datasets on average by 1.4\% and 1.7\% respectively. 2) Since our summarization strategy can achieve average summary ratio of 7.42\% and though we construct two stages including summarization and knowledge-augmented generation, due to the reason that the inference cost of LLMs is linearly correlated with token number, the average inference cost increased by our approach is the cost of query itself and the summarization, we believe it's controllable. Beside, with high-quality document summary , we can further utilize it for boosting the performance and decreasing the inference cost in knowledge-intensive situations for powerful commercial LLMs such as GPT4.  

We find that the findings of the combination of summary and raw retrieved results could achieve better performance in previous research is interesting indeed, and we would like to carry out some experiments by combining these info for downstream tasks and we want to know if we can combine the conciseness of summary and the info-richness of retrieval and in the meantime with cost guarantee.

\noindent \textbf{Comment 3} The proposed method in this paper, though overall reasonable, seems to be a bit ad hoc to me. I think it is possible that, if designed in a more principled way, the authors don’t need as many components, as many training procedures to fix the retriever and LLM mis-match problem. The proposed method, although outperforms baselines, is significantly more complex. We know that LLM can achieve better performance with multiple steps of reflection, self-critique. So I am not 100\% convinced that the comparison is fully fair (given the different number of infer steps, computational cost, etc.)

\noindent \textbf{Response 3} Thank you for your comments and we would like to address your concerns from the following perspectives: 

\noindent 1) Compared to the traditional RAG pipeline that first retrieve top-k documents from hundreds of thousands document corpus using an off-the-shelf retriever, then prepend the top-k documents to the input prompt, finally call an LLM (\eg Llama) for the final answer.
If we are using the same LLM for the final answer, since the model training process tend to be one-time with a fixed cost, we only discuss the inference costs here. 
Our approach would introduce some additional cost by 
i) introducing the utility model for ranking the top-k documents from the retriever, 
ii) introducing a summarizer for abstracting information from multiple documents. 
However, we argue that comparing to retrieving top-k documents from hundreds of thousands document corpus, the cost for ranking the top-k documents using a utility model is negligible. As for the cost brought by the summarizer, since our summarization strategy can achieve average summary ratio of 7.42\%, though we construct two stages including summarization and knowledge-augmented generation, due to the reason that the inference cost of LLMs is linearly correlated with token number, the average inference cost increased by our approach is the cost of query itself and the summarization, we believe it is controllable. 

\noindent 2) With improved document set and corresponding high-quality document summary, we can further utilize it for boosting the performance and decreasing the inference cost in knowledge-intensive situations for powerful commercial LLMs such as GPT4. However, for the traditional RAG pipeline, since a dozen of documents can sometimes confuse the LLM, it might need to incorporate more powerful LLMs than Llama we utilized for performance guarantee.

\noindent \textbf{Comment 4} I would encourage the authors to solidify this paper with either more convincing arguments (with citations), or with more comprehensive comparisons. Also some analysis on the computational cost, efficiency of the proposed system (compared with existing ones) would be very helpful.

\noindent \textbf{Response 4} Thank you for your nice suggestions and we will work hard to improve our paper in the following ways: 1) besides the explanations for above comments, for significant statements or motivations, we would cite more influential papers to solidify our statements, 2) to address your concerns about the efficiency, on the one hand we would like to conduct some computational cost analysis, on the other hand we would keep on improving our work by trying different ways for incorporating various techniques to achieve our goals, in order to determine if we can both improve efficiency and effectiveness.

